Online Primal Dual Meets Online Matching with Stochastic Rewards: Configuration LP to the Rescue

Mehta and Panigrahi (FOCS 2012) introduce the problem of online matching with stochastic rewards, where edges are associated with success probabilities and a match succeeds with the probability of the corresponding edge. It is one of the few online matching problems that have defied the randomized online primal dual framework by Devanur, Jain, and Kleinberg (SODA 2013) thus far. This paper unlocks the power of randomized online primal dual in online matching with stochastic rewards by employing the configuration linear program rather than the standard matching linear program used in previous works. Our main result is a 0.572 competitive algorithm for the case of vanishing and unequal probabilities, improving the best previous bound of 0.534 by Mehta, Waggoner, and Zadimoghaddam (SODA 2015) and, in fact, is even better than the best previous bound of 0.567 by Mehta and Panigrahi (FOCS 2012) for the more restricted case of vanishing and equal probabilities. For vanishing and equal probabilities, we get a better competitive ratio of 0.576. Our results further generalize to the vertex-weighted case due to the intrinsic robustness of the randomized online primal dual analysis.

==> solve-de.tex <==
\section{Solving the Differential Inequalities}
\label{sec:solve-de}

\subsection{Differential Inequality in Section~\ref{sec:equal-probabilities}}
\label{subsec:solve-de-1}

We show that how we derive $f'(x)$ in Eqn. (\ref{eqn:f-equal}) from the differential inequality in Eqn. (\ref{eqn:de-equal}). 
We need to find a $f(x)$ satisfies the following two inequalities:\\
    When $p_u(S) \geq \ell_u^{\infty}$,
    \begin{dmath}
    \label{eqn:solve-de-equal-p>l}
        \int_0^{\ell_u^\infty} e^{-\theta_u} f(\theta_u) d\theta_u + \left( e^{-\ell_u^{\infty}} p_u(S) + \int_0^{\ell_u^{\infty}} e^{-\theta_u} \big( p_u(S) - (\ell_u^{\infty}-\theta_u) \big) d\theta_u \right) \big( 1 - f(\ell_u^{\infty}) \big) 
        \geq \Gamma \cdot p_u(S);
    \end{dmath}
    When $p_u(S) < \ell_u^{\infty}$,
    \begin{dmath}
    \label{eqn:solve-de-equal-p<l}
        \int_0^{\ell_u^\infty} e^{-\theta_u} f(\theta_u) d\theta_u + \left( e^{-\ell_u^{\infty}} p_u(S) + \int_{\ell_u^{\infty}-p_u(S)}^{\ell_u^{\infty}} e^{-\theta_u} \big( p_u(S) - (\ell_u^{\infty}-\theta_u) \big) d\theta_u \right) \big( 1 - f(\ell_u^{\infty}) \big) 
        \geq \Gamma \cdot p_u(S);
    \end{dmath}
    For Eqn.(\ref{eqn:solve-de-equal-p>l}), if we fix $\ell_u^{\infty}$ and view it as a linear function of $p_u(S)$, we observe that $p_u(S)=1$ gives a lower bound of LHS in Eqn.(\ref{eqn:solve-de-equal-p>l}), since the coefficient of $p_u(S)$ is $1-f(\ell_u^{\infty}) - \Gamma$, which is at most $0$ if for any $\ell_u^{\infty} \geq 0$,
    $$1-f(\ell_u^{\infty}) \leq 1-f(0) \leq \Gamma$$
    , which simplifies Eqn.(\ref{eqn:solve-de-equal-p>l}) by set $p_u(S) =1$.
    
    To further simplify Eqn.(\ref{eqn:solve-de-equal-p>l}), we observe that it suffices to set $f(x) = 1-1/e$ when $x \geq 1$. And then if we take the derivative of both sides, Eqn.(\ref{eqn:solve-de-equal-p>l}) becomes:
    \begin{dmath}
        (-2+\ell_u^{\infty} + e^{\ell_u^{\infty}})f'(\ell_u^{\infty}) + f(\ell_u^{\infty}) = 1-e^{\ell_u^{\infty}},
    \end{dmath}
    where $L_i^{\infty} \leq 1$. Then $f(x)$ in Eqn.(\ref{eqn:f-equal}) is exactly a solution by solving the above differential equation with the boundary condition $f(1) = 1 -1/e$.
    
    For Eqn.(\ref{eqn:solve-de-equal-p<l}), similar observation shows $P_i(S)=1$ gives a lower bound of LHS. Then Eqn.(\ref{eqn:solve-de-equal-p<l}) becomes,
    \begin{dmath}
        \int_0^1 e^{-\ell_u^{\infty}}f(\ell_u^{\infty})d\ell_u^{\infty} + \frac{1}{e} - \frac{1}{e^2} \geq \Gamma,
    \end{dmath}
    where $\ell_u^{\infty} > 1$. One can easily verify the above inequality holds with equality under $f(x)$ in Eqn.(\ref{eqn:f-equal}). 
    
    Thus $\Gamma \leq 1 -f(0) \approx 0.576102$. 


\subsection{Differential Inequality in Section~\ref{sec:unequal-probabilities}}
\label{subsec:solve-de-2}

We show how we solve the differential inequality in Eqn.(\ref{eqn:de-unequal}). Similar to the equal-probabilities case, we first observe that fix $\ell_u^{\infty}$, $p_u(S)$ gives worst cases of LHS in Eqn.(\ref{eqn:de-unequal}) if,
$$1-f(\ell_u^{\infty}) \leq 1-f(0) \leq \Gamma$$
, and we can set $f(x) = 1 -1/e$ when $x \geq 1$ for further simplification. Observe that when $\ell_u^{\infty}$ is small, say, close to 0, $1-f(\ell_u^{\infty}) \geq \int_{\theta_u}^{\ell_u^{\infty}} \big( 1-f(y) \big) dy$ for $\theta_u \leq \ell_u^{\infty}$. Thus we solve the following differential inequality. 
\begin{dmath}
    \label{eqn:solve-de-unequal-1}
    \int_0^{\ell_u^\infty} e^{-\theta_u} f(\theta_u) d\theta_u
    + e^{-\ell_u^{\infty}} \big(1-f \big(\ell_u^{\infty} \big) \big)
    + \int_0^{\ell_u^{\infty}} \left(  1-f(\ell_u^{\infty}) - \int_{\theta_u}^{\ell_u^{\infty}} \big( 1-f(y) \big) dy \right) e^{-\theta_u} d\theta_u
    \geq \Gamma
\end{dmath}

Eqn.(\ref{eqn:solve-de-unequal-1}) is equivalent to
\begin{dmath}
        2-f(\ell_u^{\infty}) + \int_0^{\ell_u^{\infty}}f(z)dz - \ell_u^{\infty} - e^{-\ell_u^{\infty}}  
        \geq \Gamma
\end{dmath}
. $f(x)$ in Eqn.(\ref{eqn:f-unequal}) is a solution with a the boundary condition $f(1) =1-1/e$. One can easily verify that $f(x)$ in Eqn.(\ref{eqn:f-unequal}) satisfies Eqn.(\ref{eqn:de-unequal}) and keeps the monotonicity we need of $f(x)$, Thus $\Gamma = 1-f(0) = \frac{1}{2}(1+e^{-2}) \approx 0.567$.
